Modelling an Ammonium Transporter with SCLS

The Stochastic Calculus of Looping Sequences (SCLS) is a recently proposed modelling language for the representation and simulation of biological systems behaviour. It has been designed with the aim of combining the simplicity of notation of rewrite systems with the advantage of compositionality. It also allows a rather simple and accurate description of biological membranes and their interactions with the environment. In this work we apply SCLS to model a newly discovered ammonium transporter. This transporter is believed to play a fundamental role for plant mineral acquisition, which takes place in the arbuscular mycorrhiza, the most wide-spread plant-fungus symbiosis on earth. Due to its potential application in agriculture this kind of symbiosis is one of the main focuses of the BioBITs project. In our experiments the passage of NH3 / NH4+ from the fungus to the plant has been dissected in known and hypothetical mechanisms; with the model so far we have been able to simulate the behaviour of the system under different conditions. Our simulations confirmed some of the latest experimental results about the LjAMT2;2 transporter. The initial simulation results of the modelling of the symbiosis process are promising and indicate new directions for biological investigations.

==> eptcsdata.tex <==
\providecommand{\event}{R.J.Back, I.Petre, E. de Vink (Eds.): Computational\\
Models for Cell Processes (CompMod 2009)}
\providecommand{\volume}{6}
\providecommand{\anno}{2009}
\providecommand{\firstpage}{77}
\providecommand{\eid}{6}
\pdfoutput=1

